BertNet: Harvesting Knowledge Graphs with Arbitrary Relations from Pretrained Language Models

It is crucial to automatically construct knowledge graphs (KGs) of diverse new relations to support knowledge discovery and broad applications. Previous KG construction methods, based on either crowdsourcing or text mining, are often limited to a small predefined set of relations due to manual cost or restrictions in text corpus. Recent research proposed to use pretrained language models (LMs) as implicit knowledge bases that accept knowledge queries with prompts. Yet, the implicit knowledge lacks many desirable properties of a full-scale symbolic KG, such as easy access, navigation, editing, and quality assurance. In this paper, we propose a new approach of harvesting massive KGs of arbitrary relations from pretrained LMs. With minimal input of a relation definition (a prompt and a few shot of example entity pairs), the approach efficiently searches in the vast entity pair space to extract diverse accurate knowledge of the desired relation. We develop an effective search-and-rescore mechanism for improved efficiency and accuracy. We deploy the approach to harvest KGs of over 400 new relations from different LMs. Extensive human and automatic evaluations show our approach manages to extract diverse accurate knowledge, including tuples of complex relations (e.g., "A is capable of but not good at B"). The resulting KGs as a symbolic interpretation of the source LMs also reveal new insights into the LMs' knowledge capacities.

==> sections/experiment_backup.tex <==
We validate the effectiveness of the proposed knowledge harvesting framework with extensive experiments. 
We conduct human evaluation of our outcome KGs, and illustrate the effectiveness of the automatically created prompts in our framework. 
Besides, using our framework as a tool to interpret the LM knowledge storage, we make interesting observations about several knowledge-related questions on the black-box LMs.

We will release the whole family of extracted KGs, as well as the code implementation of our framework (included in the supplementary materials), upon acceptance.

\subsection{Setup}
\label{sec:setup}
\paragraph{Relations} 
We extract knowledge about a large diverse set of relations. We collect relations from two existing knowledge repositories, and also test on a set of new relations not included in existing KGs. Specifically, our relations include
(1) \textbf{ConceptNet} \cite{Speer2017ConceptNet5A} is one of the most popular commonsense KGs and is widely used for evaluating knowledge extraction. 
Following \cite{li-etal-2016-commonsense}, we filter the KG and subsample a set of 20 common relations (e.g. \texttt{has\_subevent}, \texttt{motivated\_by\_goal}).
The initial prompts for the relations are from the ConceptNet repository, and we randomly sample seed entity pairs from the ConceptNet KG for each relation.
(2) \textbf{LAMA} \cite{Petroni2019LanguageMA} is a popular benchmark for factual probing, containing knowledge tuples from multiple sources. Following the recent work \cite{Jiang2020HowCW, Shin2020ElicitingKF, Zhong2021FactualP}, we use the T-REx split 41 Wikipedia relations, such as \texttt{capital\_of}, \texttt{member\_of}). For each relation, the human-written prompt provided in \cite{Petroni2019LanguageMA} is used as the initial prompt and we randomly sample seed entity pairs for each relation. 
(3) \textbf{New Relations}: 
To test the flexibility of our framework for harvesting novel knowledge, we write 12 new relations of interests that can hardly be found in any existing KGs, and manually write initial prompts and seed entity pairs for them.
The resulting relations include complex relations as described in \S\ref{sec:complex}.

%More details, e.g., initial prompts, and seed entities of relations, can be found in the appendix.

\paragraph{Hyperparameters} 
\label{para:hparam}
We use 5 seed entity pairs for each relation. 
To automatically collect prompts (\S\ref{sec:search_prompts}), we use GPT-3 with the instruction \texttt{"paraphrase:\{sentence\}"} as the off-the-shelf paraphraser. In the entity pair searching (\S\ref{sec:search_ep}), we restrict every entity to appear no more than 10 times to improve the diversity of generated knowledge and search out at most 50,000 entity tuples for each relation. We finally use various scoring thresholds to get the outcome KGs in different scales, including (1) \textbf{50\%}: taking a half of all searched-out entities with higher consistency (Eq. \ref{eqn:consistent}).  (2) \textbf{base-k}: Naturally there are different numbers of valid tuples for different relations (e.g. tuples of \textsc{CapitalOf} should not exceed 200 as that is the number of all the countries in the world). We design a relation-specific thresholding method, that is to set 10\% of the $k$-nd consistency as the threshold (i.e., $0.1 * \text{consistency}_k$), and retain all tuples with consistency above the threshold. We name the settings \textbf{base-10} and \textbf{base-100} when k is 10 and 100, respectively. 
% \hsb{Where should we mention top-100 used in table 3/4?}



% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{figs/example-v4.pdf}
%     \vspace{-15pt}
%     \caption{Examples of knowledge tuples harvested from \textsc{DistillBert} (Randomly sampled).}
%     \label{fig:examples}
%     \vspace{-16pt}
% \end{figure}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figs/example-v5.pdf}
    \caption{Examples of knowledge tuples harvested from \textsc{DistillBert} (Randomly sampled). The first 7 rows shows relations with two entities (head and tail) and last 3 rows shows more complex relations with 3 entities.}
    \label{fig:examples}
\end{figure*}

\begin{table*}[t]
% \begin{wraptable}{r}{0.7\textwidth}
% \vspace{-10pt}
\centering
% \begin{minipage}{0.7\textwidth}
\begin{tabular}{@{}l l l l c c@{}}
\toprule
{\bf Method} & {\bf Relations}  & {\bf Tuple} & {\bf Diversity} & {\bf Novelty\%} & {\bf Acc\%} \\
\midrule
WebChild & 20 & 4,649,471 & - & - & 82.0$^*$\\
ASCENT & - & 8,600,000 & - & - & 79.2$^*$\\
TransOMCS & 20 &18,481,607 & 100,659 & 98.3 & 56.0$^*$\\
TupleKB & 1009 	$^\blacktriangle$ & 282,594 & 28,078 & - & -\\
Quasimodo & 6084 $^\blacktriangle$ & 2,262,109 & 80,145 & - & - \\
\midrule
% COMET$^{\text{cn}}_{\text{base-10}}$&6,741 & 4,342 & 35.5 & 92.0\\ % \midrule
COMET$^{CN}_{base\text{-}10}$&&6,741 & 4,342 & 35.5 & 92.0\\[2pt] % \midrule
% COMET$^{\text{cn}}_{\text{50\%}}$ & 230,028 & 55,350 & 72.4 & 66.6 \\ 
COMET$^{CN}_{50\%}$ && 230,028 & 55,350 & 72.4 & 66.6 \\ 
\midrule
% \textsc{RobertaNet}$^{\text{cn}}_{\text{base-10}}$ & 6,741& 6,107 & 64.4 & 88.0 \\
\textsc{RobertaNet}$^{CN}_{base\text{-}10}$ && 6,741& 6,107 & 64.4 & 88.0 \\[2pt]

% \textsc{RobertaNet}$^{\text{cn}}_{\text{base-100}}$ & 24,375& 12,762 & 68.8 & 81.6 \\
\textsc{RobertaNet}$^{CN}_{base\text{-}100}$ && 24,375& 12,762 & 68.8 & 81.6 \\[2pt]
% \textsc{RobertaNet}$^{\text{cn}}_{\text{50\%}}$ & 23,0028& 80,525  & 87.0 & 55.0 \\ 
\textsc{RobertaNet}$^{CN}_{50\%}$ && 230,028& 80,525  & 87.0 & 55.0 \\
\midrule
\textsc{RobertaNet}$^{New}_{base\text{-}10}$ && 2,180& 3,137 & - & 81.8 \\[2pt]

% \textsc{RobertaNet}$^{\text{cn}}_{\text{base-100}}$ & 24,375& 12,762 & 68.8 & 81.6 \\
\textsc{RobertaNet}$^{New}_{base\text{-}100}$ && 7,329&
6,559 & - & 68.6 \\[2pt]
% \textsc{RobertaNet}$^{\text{cn}}_{\text{50\%}}$ & 23,0028& 80,525  & 87.0 & 55.0 \\ 
\textsc{RobertaNet}$^{New}_{50\%}$ && 23,666  & 16,089 &-& 58.6 \\
\bottomrule
\end{tabular}


\setlength{\abovecaptionskip}{10pt}
\captionof{table}{Statistics of KGs constructed with different methods. \hsb{move our result to the top}
\textit{Diversity} refers to the number of unique entities in a KG, and \textit{Novelty} refers to the proportion of entities that don't appear in ConceptNet. The acceptance rate with $^*$ are from the original papers and subject to different evaluation protocol. The relation numbers marked with $^\blacktriangle$ are verb phrases populated from raw text sources and not human specified. Given COMET can only predict the tail entity given a source entity and a relation, we generate KGs with COMET by feeding it the head entity and relation of our RobertaNet. The first two blocks of this table corresponds to the first two blocks in Table \ref{tab:summary}, which includes five text-based KG construction methods: WebChild \cite{tandon2014webchild}, ASCENT \cite{nguyen2021refined}, TransOMCS \cite{Zhang2020TransOMCSFL}, TupleKB \cite{mishraDomainTargetedHighPrecision2017}, and Quasimodo \citep{romero2019commonsense}} 
\label{tab:stats}
% \end{minipage}
\vspace{-10pt}
% \end{wraptable}  
\end{table*}


\subsection{Evaluation}

\subsubsection{Evaluating outcome KGs}
We apply our framework to extract knowledge graph of \textbf{ConceptNet} (CN) relations and \textbf{New} relations from language models, and then conduct human evaluation on the accuracy of the extracted knowledge with Amazon MTurk. The correctness of each extracted knowledge tuple is labeled by 3 annotators with True/False/Unjudgeable. A tuple would be "accepted" (acc) if at least 2 annotators think it is true knowledge, and "rejected"
(rej) if at least 2 annotators rate it as false. We provide more details of human evaluation in the appendix. 

The statistics of the generated KGs from our framework (\textsc{RobertaNet}) and other knowledge extraction methods are mentioned in Table \ref{tab:stats}, and the samples of the extracted KG from \textsc{DistillBERT} can be found in Figure \ref{fig:examples}.
The acceptance rate, indicating the precision of KGs, in Table \ref{tab:stats} are \textit{not comparable} to each other, and only serves for a rough sense. 
From those statistics, we can see that with solely the LM as the knowledge source, and without any training data, our framework extracts KGs with competitive accuracy. Compared to COMET, our precision is a little lower, which is expected due to the big compromise we make in the setting, and our searching constraints ensure better diversity and novelty of \textsc{RoBERTaNet} over COMET.
% \textcolor{red}{For each language model, we extract a knowledge graphs of 75 relations from the relation sets \textbf{ConceptNet}, \textbf{LAMA}, and \textbf{New Relations}. We searched for 1000 tuples for each relations, and show the basic statistics of the knowledge graph harvested from \textsc{Roberta-large}. We would like to emphasize this KG is only an example, as it is easy to be extended by adding any user input relations and allowing more tuples in the searching steps.}

% \textcolor{red}{In Table \ref{tab:stats}, we report the size of harvested KG, i.e. the number of tuples. Since machine generated contents can be repetitive, we also report the
% number of unique words used, following \citet{west2021symbolic}. The harvested knowledge covers diverse vocabulary, because our searching strategy encourage diverse entities. We also compare the generated KG with the available knowledge in ConceptNet and LAMA, following \citet{Zhang2020TransOMCSFL}. Most of the tuples are not presented in the existing KGs (checked with strict string match), indicating the generated knowledge is novel.}

% The top concern about the harvested KGs is their accuracy. 

% With the human evaluation, we want to explore two questions: (1) how will the prompts generation methods influence knowledge accuracy? (2) what are the difference of knowledge contained in different language models?

\subsubsection{Evaluating automatic prompt creation}

To evaluate the effect of our automatic creation of prompts, we compare the generated KGs under these settings of prompts on the human-written new relations: (1) \textbf{Multi-Prompts} refers to the the full framework described in \S\ref{sec:methods} which use the automatically created diverse prompts in knowledge search. (2) \textbf{Top-1 Prompt}: To ablate the effect of ensembling multiple prompts, we evaluate the variant that uses only the prompt with largest weight (\S\ref{sec:search_prompts}) for knowledge extraction.
(3) \textbf{Human Prompt}: To further understand the effectiveness of the automatically created prompts, we assess the variant that uses the initial prompt (typically written by human) of each relation. (4) \textsc{\bf AutoPrompt} \cite{Shin2020ElicitingKF}, which was proposed to learn prompts by optimizing the likelihood of tail entity prediction on the training set. To fit in our setting, we adapt it to optimize the compatibility score (Eq.\ref{eqn:pem}) on the seed entity pairs. 
We omit other prompt tuning work \cite[e.g.,][]{Zhong2021FactualP, Qin2021LearningHT} because they either are difficult to fit in our problem or require more training data and fail with only the few shot of seed entity pairs in our setting.


The human-annotated accuracy is shown in Table \ref{tab:human_setting}.
Our \textsc{Top-1 Prompt} significantly improves the accuracy up to 9\% over the \textsc{Human Prompt}, indicating our prompt searching algorithm can produce high quality prompts. \textsc{Multi-Prompts} further improves the accuracy by around 4\%, which means the combination of diverse prompts better capture the semantics of a relation. The method using the optimized prompt by \textsc{AutoPrompt} gives a lower accuracy than the one with the human or searched prompt, because the small set of seed knowledge tuples are insufficient for learning effective prompts for the desired relations.

\begin{figure}
\begin{minipage}{0.45\textwidth}
\includegraphics[width=0.95\textwidth]{figs/curve_conceptnet.pdf}
\vspace{-8pt}
\captionof{figure}{Precision-recall on ConceptNet relations.}
\label{fig:curve_cn}

\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
\includegraphics[width=0.95\textwidth]{figs/curve_lama.pdf}
\vspace{-8pt}
\captionof{figure}{Precision-recall curve on LAMA relations. 
% \todo{Delete LPAQA-MP/P} 
}
\label{fig:curve_lama}
\end{minipage}
% \hfill
% \begin{minipage}{0.32\textwidth}
% \includegraphics[width=\textwidth]{figs/ConceptNet+LAMA_20 prompts_temp1.0.png}
% \captionof{figure}{Knowledge identification - ConceptNet}
% \end{minipage}

\end{figure}


\begin{figure}
\begin{minipage}{0.48\textwidth}
\small
\centering
\begin{tabular}{@{}r c c}
\toprule
Methods & Acc  & Rej \\ \midrule
%\textsc{Autoprompt}           & 33.14\%          &  47.21\%  \\
%Human-written Prompt & 59.93\%           & 26.71\%   \\
%Top-1 Prompt (Ours)    & 69.00\%            &  22.74\% \\
%Multiple Prompts (ours) & \textbf{72.50\%} &    \textbf{19.71\%}  
\textsc{Autoprompt}           & 0.33     &  0.47  \\
\textsc{Human Prompt} & 0.60        &0.27   \\
\textsc{Top-1 Prompt} (Ours)    & 0.69   &  0.23 \\
\textsc{Multi Prompts} (Ours) &\textbf{0.73} & \textbf{0.20}  

\\ \bottomrule
\end{tabular}
\captionof{table}{The portions of accepted and rejected tuples in human evaluation across settings, with the \textsc{RoBERTa-large} as the LM.}
\label{tab:human_setting}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\small
\centering
\begin{tabular}{@{}r c c}
\toprule
Source LMs         &Acc & Rej \\ \midrule
%\textsc{DistilBertNet}    & 67.21\%    & 23.57\%     \\
%\textsc{BertNet}$_{\text{base}}$     & 63.14\%    & 26.07\%     \\
%\textsc{BertNet}$_{\text{large}}$    & 70.07\%    & 21.86\%     \\
%\textsc{RoBERTaNet}$_{\text{base}}$  & 69.64\%    & 21.64\%     \\
%\textsc{RoBERTaNet}$_{\text{large}}$ & 72.50\%    & 19.71\%     \\
\textsc{DistilBert}    & 0.67    & 0.24     \\
\textsc{Bert-base}    & 0.63    & 0.26     \\
\textsc{Bert-large}  & 0.70    & 0.22     \\
\textsc{RoBERTa-base} & 0.70    & 0.22     \\
\textsc{RoBERTa-large}& 0.73    & 0.20     \\ \bottomrule
\end{tabular}
\vspace{-6pt}
\captionof{table}{The portions of accepted and rejected tuples in human evaluation across different LMs, using the \textsc{Multi-Prompts} approach.}
\label{tab:human_model}
\end{minipage}
\vspace{-15pt}
\end{figure}

Based on the results above, we move a step forward to see how the created prompts influence the subsequent module in the framework.
Specifically, we evaluate if the automatically created prompts (\S\ref{sec:search_prompts}) bring the consistency scoring (\S\ref{sec:search_ep}) better balance of knowledge accuracy (precision) and coverage (recall), by comparing various scoring methods on existing terms in ConceptNet and LAMA dataset. To be more detailed, we use the knowledge tuples from ConceptNet and LAMA as positive samples (\S\ref{sec:setup}), and synthesize the same amount of negative samples with the same strategy in \cite{li-etal-2016-commonsense} by random replacing entities or relations in the true knowledge. 
Each evaluated method estimates a score of each sample being positive (i.e., true knowledge), and ranks the samples based on the scores. We can then compute both the \emph{precision} and \emph{recall} of positive samples at different cut-off points along the ranking, and plot the precision-recall curves for each method.
% (we average the precision of different relations at the same recall, i.e., macro-average). 

The automatic evaluation setting on given knowledge terms also enables us to adapt existing prevalent works, e.g., KG completion and factual probing (Table~\ref{tab:summary}), for comparison with our approach:
{\bf (1)} \textsc{\bf COMET} \cite{Bosselut2019COMETCT} is a transformer-based KG completion model trained to predict the tail entity $t$ conditioning on the head entity and relation $(h, r)$ on ATOMIC \cite{Sap2019ATOMICAA}. The model has encoded rich commonsense knowledge. We thus test it on the ConceptNet commonsense data, and use its log-likelihood $\log P(t|h, r)$ as the score for each given knowledge tuple.
% Since COMET is trained to predict the tail entity $t$ conditioning on the head entity and relation $(h, r)$, we use COMET to calculate the log-likelihood $\log P(t|h, r)$ as its score function for a given candidate knowledge tuple $(h, r, t)$.
{\bf (2)} \textsc{\bf LPAQA} \cite{Jiang2020HowCW} collects a set of prompts on LAMA with text mining and paraphrasing, and ensembles them to optimize the factual probing task (and thus cannot extract new knowledge like ours). We report the best performance of its three variants. 

The resulting precision-recall curves on ConceptNet and LAMA knowledge are shown in Figure~\ref{fig:curve_cn} and Figure~\ref{fig:curve_lama}, respectively.
The variant of our \textsc{Top-1 Prompt} from our automatically-collected prompt set is significantly better than the \textsc{Human Prompt}. 
This is because the human-written prompts often fail to effectively account for possible ambiguities in the expression, which are eliminated in our approach by leveraging the seed entity pairs with compatibility measure.
%, while the creation of prompts in our framework makes use of the information in seed entity pairs.
% We conclude that's because people don't consider whether expected knowledge will be fitted into the written prompt grammatically, and don't know what prompt is good for LMs \cite{elazar2021}, while the prompts searched with $PEM$ score is good at them. 
Increasing the number of prompts (\textsc{Multi-Prompts}) provides further improvements, showing the multiple automatically created prompts can represent the desired relations more accurately and better guide the LMs for consistency. 
Our approach also substantially outperforms other baselines, like \textsc{Comet} on ConceptNet and \textsc{LPAQA} on LAMA, indicating better knowledge correctness (precision) and coverage (recall) of our framework in the context. On both datasets, \textsc{AutoPrompt}, with only 5 seed entity pairs as its training data, gives inferior performance than other approaches, indicating that the current prompt optimization is not feasible for discovering knowledge of new relations without large training data.
% Our framework also outperforms COMET on ConceptNet and LPAQA on LAMA, showing our $PEM$ is a better objective than those used for factual probing and knowledge graph completion) in our setting. 
%which means the prompts by our searching are precisely represent the given relation regarding the language model. \hzt{All the model names are obsolete..} 
%\hzt{There are two figures. Are the conclusions exact the same? If so, explicitly say that. If not, talk about it and give intuitive explanations.} %\hzt{The two figures have different baselines, explain it briefly.}
 

% \begin{table}[t]
%     \centering
%     \begin{tabular}{@{}ll|l@{}}
% \toprule
% \multicolumn{2}{l|}{Definitive prompt}                & Seed entity pairs                     \\ \midrule
% \multicolumn{2}{l|}{\multirow{3}{*}{A needs B to C}}  & (people, social media, connect)                       \\
% \multicolumn{2}{l|}{}                                 & (pig, food, grow)            \\
% \multicolumn{2}{l|}{}                                 & ...                                    \\ \midrule
% \multicolumn{2}{l|}{Searched-out prompts}             & Searched-out entity pairs             \\ \midrule
% 0.16     & A requires B in order to C                & (species, food resources, survive)     \\
% 0.13     & A feel that they need B in order to C     & (new children, care, cope)             \\
% 0.11     & In order to C, A need B                   & (people, money, live)                  \\
% 0.11     & A needs B to C                            & (society, more people, survive better) \\
% 0.08     & There is a need for B to C A              & (good friends, respect, stay)          \\
% ...      &                                           & ...                                    \\ \bottomrule
% \end{tabular}
%     \caption{A running example of relations with more than two entities.}
%     \label{tab:running_example}
% \end{table}




\subsection{Analysis of Knowledge in Different LMs} 
\label{sec:x-net}
% Our framework can be used as a tool to analyze the knowledge storage in language models. We conduct knowledge identification task with the best scoring function in section xxx, but with different language models, and also do human evaluation on the generated knowledge graphs based on several language models.

As discussed in \S\ref{sec:methods}, the outcome knowledge graphs can be treated as a fully symbolic interpretation of pretrained language models. We use \textsc{Multi-Prompts} to harvest KGs from 5 different LMs and evaluate them with human annotation. The results are shown in Table \ref{tab:human_model}, which sheds some new light on 
%\hzt{This statement is overly confident and can easily be challenged by reviewers. Use softer tone.} 
several knowledge-related questions regarding the LMs' knowledge capacity.

{\bf Does a larger LM encode better knowledge?} For BERT (and RoBERTa), the large version and the base version share the same pretraining corpus and tasks, respectively, while the large version has a larger model architecture than the base version in terms of layers (24 v.s. 12), attention heads (16 v.s. 12), and the number of parameters (340M v.s. 110M). We can see that BertNet-large and RoBERTaNet-large are around 7\% and 3\% higher than their base version, separately, so the large models indeed encoded better knowledge than the base models.

{\bf Does better pretraining bring better knowledge?} RoBERTa uses the same architecture as BERT but with better pretraining strategies, like dynamic masking, larger batch size, etc. In their extracted knowledge graphs from our framework, RoBERTaNet-large performs better than BertNet-large (0.73 v.s. 0.70), and RoBERTaNet-base is also better than BertNet-base (0.70 v.s. 0.63), which indicates the better pretraining indeed bring the better knowledge learning and storage.

{\bf Is knowledge really kept in the knowledge distillation process?} DistilBERT is trained by distilling BERT-base, and reduces 40\% parameters from it. Interestingly, the knowledge distillation process instead improves around 4\% of accuracy in the result knowledge graph. This might be because the knowledge distillation is able to remove some noisy information from the teacher model.





%\hzt{We have a whole subsection in Method to highlight that we can do complex relations. But in experiments, we just very briefly mention this in this single sentence.. We shall write more to highlight the results (and that previous methods are not capable of doing it), give example outputs, so that the paper reads more interesting.}

